Simultaneously Transmitting and Reflecting (STAR)-RISs: Are they Applicable to Dual-Sided Incidence?

A hardware model and a signal model are proposed for dual-sided simultaneously transmitting and reflecting reconfigurable intelligent surfaces (STAR-RISs), where the signal simultaneously incident on both sides of the surface. Based on the proposed hardware model, signal models for dual-sided STAR-RISs are developed. For elements with scalar surface impedance, it is proved that their transmission and reflection coefficients on both sides are identical. Based on the obtained symmetrical dual-sided STAR model, a STAR-RIS-aided two-user uplink communication system is investigated for both non-orthogonal multiple access (NOMA) and orthogonal multiple access (OMA) schemes. Analytical results for the outage probabilities for users are derived in the high transmit signal-to-noise ratio (SNR) regime. Numerical results demonstrate the performance gain of NOMA over OMA and reveal that the outage probability error floor can be lowered by adjusting the ratio between the amplitudes of transmission and reflection signals.

==> others.tex <==
\section{Mac Control}
\begin{figure}[h!]
    \begin{center}
        \includegraphics[scale=0.07]{mac_fig/MAC_RIS.jpg}
        \caption{STAR-RIS as a medium access controller for RF resources.}
        \label{sys1}
    \end{center}
\end{figure}
\begin{itemize}
    \item For wireless communications through the RF medium, there is a scarcity of medium access control. In today's communication system, transceivers of different applications shares the same physical transmission medium. Moreover, the medium is only divided into different cells based on physical distances or different frequency bands based on the carrier frequencies and bandwidths. However, due to the increased number or mobile devices, more and more terminals need to be accommodated within the urban area. In the same time, new wireless technologies are emerging which may take up more RF resource, such as RF sensing network for IoT, UAV local networks, and ...\\
    Consequently, there is a increasing need for a medium access controller to mitigate interference and collisions of the wireless channels.
\end{itemize}




%%%%%%%%%%
\begin{comment}
\begin{figure*}[t!]
\centering
\subfigure[Time-Switching]{\label{sysa}
\includegraphics[width= 2in]{mac_fig/sys_a.eps}}
\subfigure[Unicast]{\label{sysb}
\includegraphics[width= 2in]{mac_fig/sys_b.eps}}
\subfigure[Multicast]{\label{sysc}
\includegraphics[width= 2.2in]{mac_fig/sys_c.eps}}
\caption{Illustration of the working modes of the full-duplex STAR-RISs}\label{nice}
\end{figure*}

As shown in Fig.~\ref{sysa}, for the time-switching double-sided unicast scenario, Tx1 and Tx2 transmit their signals to their corresponding receivers in separate time slots. In the first time slot, Tx1 sends message $s_1$ to Rx1, and the $m$th element is configured to transmit $s_1$ from \textit{Space A} to \textit{Space B} with transmission coefficient $T^{A,B}_m$. Similarly, in the second time slot, $s_2$ is transmitted from \textit{Space B} to \textit{Space A} with transmission coefficient $T^{B,A}_m$. Because $s_1$ and $s_2$ are transmitted in different time slots, $T^{A,B}_m$ and $T^{B,A}_m$ can be independently configured. To sum up, we have the following signal model for STAR-RIS:
\subsubsection*{Case 1}
For the time-switching double-sided unicast scenario, the STAR-RIS elements can be modeled using the following transmission coefficients:
\begin{equation}
    T^{A,B}_m = \beta^{A,B}_m e^{j\phi^{A,B}_m} \text{, and  } T^{B,A}_m = \beta^{B,A}_m e^{j\phi^{B,A}_m},
\end{equation}
where $\beta^{A,B}_m$ and $\beta^{B,A}_m\in [0,1]$ are the amplitudes of the corresponding transmission coefficients, $\phi^{A,B}_m$ and $\phi^{B,A}_m \in[0,2\pi)$ are the phases of the transmission coefficients in time slot 1 and 2, respectively.
\end{comment}



%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
Different from the single source case which have been previously studied, the T\&R coefficients on the two sides of the $m$th element can be defined as follows:
\begin{align}\label{tab1}
    T^{A,B}_m &= ({E}^J+{E}^K_2+{E}^{inc}_1)/{E}^{inc}_1, \\
    T^{B,A}_m &= ({E}^J+{E}^K_1+{E}^{inc}_2)/{E}^{inc}_2, \\
    R^{A}_m &= ({E}^J+{E}^K_1+{E}^{inc}_2)/{E}^{inc}_1, \\ \label{rb1}
    R^{B}_m &= ({E}^J+{E}^K_2+{E}^{inc}_1)/{E}^{inc}_2,
\end{align}
where $E^J = ||\mathbf{E}^J||_2$,  $E^K_1 = ||\mathbf{E}^K_1||_2$, $E^K_2 = ||\mathbf{E}^K_2||_2$, $E^{inc}_1 = ||\mathbf{E}^{inc}_1||_2$, and $E^{inc}_2 = ||\mathbf{E}^{inc}_2||_2$ are the magnitudes of the corresponding electric field at the $m$th element. 

\begin{theorem}\label{t1}
Given incident signals on both sides ($E^{inc}_1$ and $E^{inc}_2$), a STAR-RIS element can be modeled using the following coefficients:
\begin{align}\label{tab}
    &T^{A,B}_m = T^0_m + \beta R^0_m,\\ \label{tba}
    &T^{B,A}_m = T^0_m + (1/\beta) R^0_m,\\ \label{ra}
    &R^{A}_m = R^0_m + \beta T^0_m,\\ \label{rb}
    &R^{B}_m = R^0_m + (1/\beta) T^0_m,
\end{align}
where $T^0_m = \frac{2Z_e}{2Z_e+\eta} - \frac{Z_m}{Z_m+2\eta}$, $R^0_m = \frac{Z_m}{Z_m+2\eta}-\frac{\eta}{2Z_e+\eta}$, $\eta$ is the free space wave impedance, and $\beta = E^{inc}_2/E^{inc}_1$ is the ratio between the amplitudes of the incident electric fields.
\begin{proof}
The boundary conditions~\cite{rNGfm99RfAqifzEoqjYY9NPszcDnpChRWu} of EM field at the surface can be expressed as $\hat{z}\times (\mathbf{H}^J_2-\mathbf{H}^J_1)\hat{y} = \mathbf{J}_s\hat{x}$ and $\hat{z}\times(\mathbf{E}^K_1 - \mathbf{E}^K_2)=\mathbf{K}_s\hat{y}$. Next, by considering \eqref{js} and \eqref{ks} with the boundary conditions, $E^J$ and $E^K_1$ in \eqref{tab1}-\eqref{rb1} can be expressed in terms of $Z_e$, $Z_m$, and $\eta$, i.e., we have the following:
\begin{align}\label{tab2}
    &E^J = \frac{-\eta(E^{inc}_1+E^{inc}_2)}{2Z_e+\eta},\\ \label{tab3}
    &E^K_1 = \frac{Z_m(E^{inc}_1-E^{inc}_2))}{Z_m+2\eta}.
\end{align}
Finally, by plugging \eqref{tab2} and \eqref{tab3} into \eqref{tab1}-\eqref{rb1}, the proof is finished.
\end{proof}
\end{theorem}

\begin{remark}
In \eqref{tab}-\eqref{rb}, $T^0_m$ and $R^0_m$ are the T\&R coefficients given a one-sided signal incidence. According to existing studies~\cite{xu_star,liu_star,mu_star}, the phases of $T^0_m$ and $R^0_m$, i.e., $\phi^T_m$ and $\phi^R_m$ can be independently configured while their amplitudes are constrained through the law of energy conservation, namely:
\begin{align}
    |T^0_m|^2+|R^0_m|^2 \leq 1\\
    \phi^T_m,\ \phi^R_m \in [0,2\pi).
\end{align}
For passive lossless STAR-RIS element, $\phi^T_m$ and $\phi^R_m$ are further correlated~\cite{xu_correlated}.
\end{remark}
The physical meaning of these coefficients can be understood through \eqref{tab}-\eqref{rb}: For general cases, $T^{A,B}_m \neq T^{B,A}$, and $R^A_m \neq R^B_m$. This is due to the asymmetric strengths of incident EM waves on the two sides. In the following, we present the signal models for STAR-RISs operating in purely transmitting, purely reflecting, and simultaneous transmitting and reflecting modes.
